NeuraLoc: Visual Localization in Neural Implicit Map with Dual Complementary Features

Recently, neural radiance fields (NeRF) have gained significant attention in the field of visual localization. However, existing NeRF-based approaches either lack geometric constraints or require extensive storage for feature matching, limiting their practical applications. To address these challenges, we propose an efficient and novel visual localization approach based on the neural implicit map with complementary features. Specifically, to enforce geometric constraints and reduce storage requirements, we implicitly learn a 3D keypoint descriptor field, avoiding the need to explicitly store point-wise features. To further address the semantic ambiguity of descriptors, we introduce additional semantic contextual feature fields, which enhance the quality and reliability of 2D-3D correspondences. Besides, we propose descriptor similarity distribution alignment to minimize the domain gap between 2D and 3D feature spaces during matching. Finally, we construct the matching graph using both complementary descriptors and contextual features to establish accurate 2D-3D correspondences for 6-DoF pose estimation. Compared with the recent NeRF-based approaches, our method achieves a 3$\times$ faster training speed and a 45$\times$ reduction in model storage. Extensive experiments on two widely used datasets demonstrate that our approach outperforms or is highly competitive with other state-of-the-art NeRF-based visual localization methods. Project page: \href{https://zju3dv.github.io/neuraloc}{https://zju3dv.github.io/neuraloc}

==> figs/0_teaser.tex <==
\begin{figure}[t]
\centering
 \includegraphics[width=\linewidth]{figures/teaser.png}\\
\caption{\textbf{Localization with neual map}. \zhj{update figure} For the query image, we extract 2D descriptors and context features via pre-trained CNN models~\cite{sam,superpoint}.
For 3D points inside the frustum of the reference image, we render its 3D descriptors and context features via our implicit semantic map.
The 6 DoF pose can be obtained via PnP+RANSAC according to the 2D-3D correspondence estimated by our matching graph.}
\label{fig:teaser}
\end{figure}

==> tables/1.tex <==
%------------------------------------------------------------------------------
% 不同阶段的定位精度
%------------------------------------------------------------------------------

\begin{table}[h]
\centering
% \footnotesize
% \scriptsize
\caption{Results of retrieval initialization and our approach.}
\setlength{\tabcolsep}{5pt}
\begin{tabularx}{0.93\linewidth}{lcccc}
\toprule
Method & Room 0 & Room 1  & Office 0 & Office 1  \\
\midrule
Retrieval & 82.97,16.61 & 98.76,25.02 & 83.24,16.86 & 87.96,17.39 \\
Ours & 0.51,0.08 & 1.06,0.20 & 0.39,0.08 & 0.82,0.21\\
\bottomrule
\end{tabularx}
\label{tab:diff_stage}
\end{table}

